Molecular beam epitaxy of single crystalline GaN nanowires on a flexible Ti foil

We demonstrate the self-assembled growth of vertically aligned GaN nanowire ensembles on a flexible Ti foil by plasma-assisted molecular beam epitaxy. The analysis of single nanowires by transmission electron microscopy reveals that they are single crystalline. Low-temperature photoluminescence spectroscopy demonstrates that, in comparison to standard GaN nanowires grown on Si, the nanowires prepared on the Ti foil exhibit a equivalent crystalline perfection, a higher density of basal-plane stacking faults, but a reduced density of inversion domain boundaries. The room-temperature photoluminescence spectrum of the nanowire ensemble is not influenced or degraded by the bending of the substrate. The present results pave the way for the fabrication of flexible optoelectronic devices based on GaN nanowires on metal foils.

==> references.tex <==

@Article{Abramoff2004,
  author =  {Abramoff, M.D. and Magalh\~{a}es, P.J. and  Ram, S.J.},
  title =   {{Image processing with ImageJ}},
  journal = {Biophotonics Int.},
  year =    {2004},
  volume =  {11},
  number =  {7},
  pages =   {36--42},
  url =     {http://webeye.ophth.uiowa.edu/dept/biograph/abramoff/imagej.pdf}
}

@article{Auzelle2015,
author = {Auzelle, Thomas and Haas, Benedikt and {Den Hertog}, Martien and Rouvi\`{e}re, Jean-Luc and Daudin, Bruno and Gayral, Bruno},
doi = {10.1063/1.4927826},
issn = {0003-6951},
journal = {App. Phys. Lett.},
number = {5},
pages = {051904},
title = {{Attribution of the 3.45 eV GaN nanowires luminescence to inversion domain boundaries}},
url = {http://scitation.aip.org/content/aip/journal/apl/107/5/10.1063/1.4927826},
volume = {107},
year = {2015}
}

@Article{Bauer1990,
  author =   {Bauer, Ernst G. and Dodson, Brian W. and Ehrlich, Daniel J. and Feldman, Leonard C. and Flynn, C. Peter and Geis, Michael W. and Harbison, James P. and Matyi, Richard J. and Peercy, Paul S. and Petroff, Pierre M. and Phillips, Julia M. and Stringfellow, Gerald B. and Zangwill, Andrew},
  title =    {{Fundamental issues in heteroepitaxy—A Department of Energy, Council on Materials Science Panel Report}},
  journal =  {J. Mater. Res.},
  year =     {1990},
  volume =   {5},
  pages =    {852--894},
  doi =      {10.1557/JMR.1990.0852},
  issue =    {04},
  numpages = {43},
  url =      {http://journals.cambridge.org/article_S0884291400009377}
}

@article{Brandt2014,
author = {Brandt, Oliver and Fern\'{a}ndez-Garrido, Sergio and Zettler, Johannes K. and Luna, Esperanza and Jahn, Uwe and Ch\`{e}ze, Caroline and Kaganer, Vladimir M.},
journal = {Cryst. Growth Des.},
number = {5},
pages = {2246--2253},
title = {{Statistical Analysis of the Shape of One-Dimensional Nanostructures: Determining the Coalescence Degree of Spontaneously Formed GaN Nanowires}},
volume = {14},
url = {http://pubs.acs.org/doi/abs/10.1021/cg401838q},
year = {2014}
}

@article{Calleja2000,
author = {Calleja, Enrique and S\'{a}nchez-Garc\'{\i}a, M. and S\'{a}nchez, F. and Calle, F. and Naranjo, F. and Mu\~{n}oz, E. and Jahn, Uwe and Ploog, Klaus H.},
doi = {10.1103/PhysRevB.62.16826},
issn = {0163-1829},
journal = {Phys. Rev. B},
number = {24},
pages = {16826--16834},
title = {{Luminescence properties and defects in GaN nanocolumns grown by molecular beam epitaxy}},
url = {http://link.aps.org/doi/10.1103/PhysRevB.62.16826},
volume = {62},
year = {2000}
}

@Article{Consonni2009,
  author =        {Consonni, Vincent and Knelangen, Matthias and Jahn, Uwe and Trampert, Achim and Geelhaar, Lutz and Riechert, Henning},
  title =         {{Effects of nanowire coalescence on their structural and optical properties on a local scale}},
  journal =       {App. Phys. Lett.},
  year =          {2009},
  volume =        {95},
  number =        {24},
  pages =         {241910},
  doi =           {10.1063/1.3275793},
  issn =          {00036951},
  mendeley-tags = {PDI},
  url =           {http://link.aip.org/link/APPLAB/v95/i24/p241910/s1\&Agg=doi}
}

@Article{Corfdir2014,
  author =  {Corfdir, Pierre and Zettler, Johannes K. and Hauswald, Christian and Fern\'{a}ndez-Garrido, Sergio and Brandt, Oliver and Lefebvre, Pierre},
  title =   {{Sub-meV linewidth in GaN nanowire ensembles: Absence of surface excitons due to the field ionization of donors}},
  journal = {Phys. Rev. B},
  year =    {2014},
  volume =  {90},
  number =  {20},
  url = {http://link.aps.org/doi/10.1103/PhysRevB.90.205301},
  pages =   {205301}
}

@article{Corfdir2014b,
author = {Corfdir, Pierre and Hauswald, Christian and Zettler, Johannes K. and Flissikowski, Timur and Laehnemann, Jonas and Fern\'{a}ndez-Garrido, Sergio and Geelhaar, Lutz and Grahn, H. T. and Brandt, Oliver},
doi = {10.1103/PhysRevB.90.195309},
issn = {1098-0121},
journal = {Phys. Rev. B},
number = {19},
pages = {195309},
title = {{Stacking faults as quantum wells in nanowires: Density of states, oscillator strength, and radiative efficiency}},
url = {http://link.aps.org/doi/10.1103/PhysRevB.90.195309},
volume = {90},
year = {2014}
}

@article{Dai2015,
author = {Dai, Xing and Messanvi, Agnes and Zhang, Hezhi and Durand, Christophe and Eymery, J\"{o}el and Bougerol, Catherine and Julien, Fran\c{c}ois H. and Tchernycheva, Maria},
doi = {10.1021/acs.nanolett.5b02900},
issn = {1530-6984},
journal = {Nano Lett.},
number = {10},
pages = {6958--6964},
title = {{Flexible Light-Emitting Diodes Based on Vertical Nitride Nanowires}},
url = {http://pubsdc3.acs.org/doi/10.1021/acs.nanolett.5b02900},
volume = {15},
year = {2015}
}

@article{Fan2009,
author = {Fan, Zhiyong and Razavi, Haleh and Do, Jae-Won and Moriwaki, Aimee and Ergen, Onur and Chueh, Yu-Lun and Leu, Paul W and Ho, Johnny C and Takahashi, Toshitake and Reichertz, Lothar A and Neale, Steven and Yu, Kyoungsik and Wu, Ming and Ager, Joel W and Javey, Ali},
doi = {10.1038/nmat2493},
issn = {1476-1122},
journal = {Nat. Mater.},
keywords = {Solar Cell},
mendeley-tags = {Solar Cell},
month = aug,
number = {8},
pages = {648--653},
pmid = {19578336},
publisher = {Nature Publishing Group},
title = {{Three-dimensional nanopillar-array photovoltaics on low-cost and flexible substrates}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/19578336 http://www.nature.com/doifinder/10.1038/nmat2493},
volume = {8},
year = {2009}
}

@Article{Fernandez-Garrido2012,
  author =  {Fern\'{a}ndez-Garrido, Sergio and Kong, Xiang and Gotschke, Tobias and Calarco, Raffaella and Geelhaar, Lutz and Trampert, Achim and Brandt, Oliver},
  title =   {{Spontaneous Nucleation and Growth of GaN Nanowires: The Fundamental Role of Crystal Polarity}},
  journal = {Nano Lett.},
  year =    {2012},
  volume =  {12},
  number =  {12},
  pages =   {6119--6125},
  doi =     {10.1021/nl302664q},
  url =     {http://www.ncbi.nlm.nih.gov/pubmed/23130785}
}

@Article{Fernandez-Garrido2014,
  author =    {Fern\'{a}ndez-Garrido, Sergio and Kaganer, Vladimir M. and Hauswald, Christian and Jenichen, Bernd and Ramsteiner, M and Consonni, Vincent and Geelhaar, Lutz and Brandt, Oliver},
  title =     {{Correlation between the structural and optical properties of spontaneously formed GaN nanowires: a quantitative evaluation of the impact of nanowire coalescence}},
  journal =   {Nanotechnology},
  year =      {2014},
  volume =    {25},
  number =    {45},
  pages =     {455702},
  doi =       {10.1088/0957-4484/25/45/455702},
  issn =      {0957-4484},
  publisher = {IOP Publishing},
  url =       {http://stacks.iop.org/0957-4484/25/i=45/a=455702?key=crossref.ee03f7ad030e752a06a5b1891f62f814}
}

@article{Hersee2006,
author = {Hersee, Stephen D. and Sun, Xinyu and Wang, Xin},
title = {The Controlled Growth of GaN Nanowires},
journal = {Nano Lett.},
volume = {6},
number = {8},
pages = {1808-1811},
year = {2006},
doi = {10.1021/nl060553t},
URL = {http://dx.doi.org/10.1021/nl060553t}
}

@article{Hersee2011,
author = {Hersee, Stephen D. and Rishinaramangalam, Ashwin K. and Fairchild, Michael N. and Zhang, Lei and Varangis, Petros},
doi = {10.1557/jmr.2011.112},
issn = {0884-2914},
journal = {J. Mater. Res.},
language = {English},
month = jun,
number = {17},
pages = {2293--2298},
publisher = {Cambridge University Press},
title = {{Threading defect elimination in GaN nanowires}},
url = {http://journals.cambridge.org/abstract\_S0884291411001129},
volume = {26},
year = {2011}
}

@article{Hestroffer2011,
author = {Hestroffer, Karine and Leclere, C\'{e}dric and Bougerol, Catherine and Renevier, Hubert and Daudin, Bruno},
issn = {1098-0121},
journal = {Phys. Rev. B},
number = {24},
pages = {245302},
title = {{Polarity of GaN nanowires grown by plasma-assisted molecular beam epitaxy on Si(111)}},
url = {http://prb.aps.org/abstract/PRB/v84/i24/e245302},
volume = {84},
year = {2011}
}

@article {Kim2010,
author = {Kim, Dae-Hyeong and Xiao, Jianliang and Song, Jizhou and Huang, Yonggang and Rogers, John A.},
title = {Stretchable, Curvilinear Electronics Based on Inorganic Materials},
journal = {Advanced Materials},
volume = {22},
number = {19},
publisher = {WILEY-VCH Verlag},
issn = {1521-4095},
url = {http://dx.doi.org/10.1002/adma.200902927},
doi = {10.1002/adma.200902927},
pages = {2108--2124},
keywords = {Flexible electronics, Nanomechanics, Plastic electronics, Semiconductor nanomaterials, Stretchable electronics},
year = {2010},
}

@Article{Kumar2011,
  author =  {{Rakesh Kumar}, R. and {Narasimha Rao}, K. and Phani, A. R.},
  title =   {{Growth and characterization of germanium nanowires on a flexible aluminium substrate by electron beam evaporation}},
  journal = {Appl. Nanoscience},
  year =    {2011},
  volume =  {1},
  number =  {4},
  pages =   {211--217},
  url =     {http://link.springer.com/article/10.1007%2Fs13204-011-0029-9#/page-1}
}

@article{Lee2011,
author = {Lee, Chi Hwan and Kim, Dong Rip and Zheng, Xiaolin},
doi = {10.1021/nl201901z},
journal = {Nano Lett.},
number = {8},
pages = {3435--3439},
pmid = {21696196},
title = {{Fabrication of Nanowire Electronics on Nonconventional Substrates by Water-Assisted Transfer Printing Method}},
url = {http://pubs.acs.org/doi/abs/10.1021/nl201901z},
volume = {11},
year = {2011}
}

@article{Liu2015,
author = {Liu, Zhe and Xu, Jing and Chen, Di and Shen, Guozhen},
doi = {10.1039/C4CS00116H},
issn = {0306-0012},
journal = {Chem. Soc. Rev.},
number = {1},
pages = {161--192},
pmid = {25242346},
publisher = {Royal Society of Chemistry},
title = {{Flexible electronics based on inorganic nanowires}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/25242346 http://xlink.rsc.org/?DOI=C4CS00116H},
volume = {44},
year = {2015}
}

@Article{Luther1998,
  author =  {Luther, B P and Mohney, S E and Jackson, T N},
  title =   {{Titanium and titanium nitride contacts to n-type gallium nitride}},
  journal = {Semicond. Sci. Tech.},
  year =    {1998},
  volume =  {13},
  number =  {11},
  pages =   {1322--1327},
  doi =     {10.1088/0268-1242/13/11/017},
  isbn =    {0268-1242},
  issn =    {0268-1242},
  url =     {http://stacks.iop.org/0268-1242/13/i=11/a=017?key=crossref.cfb56653073c53fee1056295b118552e}
}

@article{Madaria2010,
author = {Madaria, Anuj R. and Kumar, Akshay and Ishikawa, Fumiaki N. and Zhou, Chongwu},
doi = {10.1007/s12274-010-0017-5},
isbn = {1998-0124},
issn = {1998-0124},
journal = {Nano Res.},
keywords = {Ag nanowire,PDMS transfer,flexible electronics,percolation network,transparent electrode},
number = {8},
pages = {564--573},
title = {{Uniform, highly conductive, and patterned transparent films of a percolating silver nanowire network on rigid and flexible substrates using a dry transfer technique}},
url = {http://link.springer.com/10.1007/s12274-010-0017-5},
volume = {3},
year = {2010}
}

@Article{Manekkathodi2010,
  author =    {Manekkathodi, Afsal and Lu, Ming-Yen and Wang, Chun Wen and Chen, Lih-Juann},
  title =     {{Direct Growth of Aligned Zinc Oxide Nanorods on Paper Substrates for Low-Cost Flexible Electronics}},
  journal =   {Adv. Mater.},
  year =      {2010},
  volume =    {22},
  number =    {36},
  pages =     {4059--4063},
  publisher = {WILEY-VCH Verlag},
  url =       {http://onlinelibrary.wiley.com/doi/10.1002/adma.201001289/abstract}
}

@Article{McAlpine2007,
  author =   {McAlpine, Michael C and Ahmad, Habib and Wang, Dunwei and Heath, James R},
  title =    {{Highly ordered nanowire arrays on plastic substrates for ultrasensitive flexible chemical sensors}},
  journal =  {Nat. Mater.},
  year =     {2007},
  volume =   {6},
  number =   {5},
  pages =    {379--384},
  pmid =     {17450146},
  url =      {http://dx.doi.org/10.1038/nmat1891 http://www.nature.com/doifinder/10.1038/nmat1891}
}

@Article{Nadarajah2008,
  author =  {Nadarajah, Athavan and Word, Robert C. and Meiss, Jan and K\"{o}nenkamp, Rolf},
  title =   {{Flexible Inorganic Nanowire Light-Emitting Diode}},
  journal = {Nano Lett.},
  year =    {2008},
  volume =  {8},
  number =  {2},
  pages =   {534--537},
  pmid =    {18220439},
  url =     {http://pubs.acs.org/doi/abs/10.1021/nl072784l}
}

@Article{Palmstrom1995,
  author =  {Palmstr{\o}m, C J},
  title =   {{Epitaxy of Dissimilar Materials}},
  journal = {Ann. Rev. Mater. Sci.},
  year =    {1995},
  volume =  {25},
  number =  {1},
  pages =   {389--415},
  doi =     {10.1146/annurev.ms.25.080195.002133},
  issn =    {0084-6600},
  url =     {http://www.annualreviews.org/doi/abs/10.1146/annurev.ms.25.080195.002133}
}

@article{Park2014,
author = {Park, Jun Beom and Kim, Nam-Jung and Kim, Yong-Jin and Lee, Sang-Hyup and Yi, Gyu-Chul},
doi = {10.1016/j.cap.2014.08.007},
issn = {15671739},
journal = {Curr. Appl. Phys.},
number = {11},
pages = {1437--1442},
title = {{Metal catalyst-assisted growth of GaN nanowires on graphene films for flexible photocatalyst applications}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S156717391400248X},
volume = {14},
year = {2014}
}

@article{Park2015,
author = {Park, Youngseo and Jahangir, Shafat and Park, Yongjun and Bhattacharya, Pallab and Heo, Junseok},
doi = {10.1364/OE.23.00A650},
issn = {1094-4087},
journal = {Opt. Express},
number = {11},
pages = {A650},
title = {{InGaN/GaN nanowires grown on SiO\_2 and light emitting diodes with low turn on voltages}},
url = {https://www.osapublishing.org/abstract.cfm?URI=oe-23-11-A650},
volume = {23},
year = {2015}
}

@article{Romanyuk2015,
author = {Romanyuk, O. and Fern\'{a}ndez-Garrido, Sergio and Jiř\'{\i}\v{c}ek, P. and Barto\v{s}, I. and Geelhaar, Lutz and Brandt, Oliver and Paskova, T.},
doi = {10.1063/1.4905651},
issn = {0003-6951},
journal = {App. Phy. Lett.},
keywords = {PDI},
mendeley-tags = {PDI},
pages = {021602},
title = {{Non-destructive assessment of the polarity of GaN nanowire ensembles using low-energy electron diffraction and x-ray photoelectron diffraction}},
volume = {106},
year = {2015}
}

@Article{Ruvimov1996,
  author =  {Ruvimov, S. and Liliental-Weber, Z. and Washburn, J. and Duxstad, K. J. and Haller, E. E. and Fan, Z.-F. and Mohammad, S. N. and Kim, W. and Botchkarev, A. E. and Morko\c{c}, H.},
  title =   {{Microstructure of Ti/Al and Ti/Al/Ni/Au Ohmic contacts for n-GaN}},
  journal = {Appl. Phys. Lett.},
  year =    {1996},
  volume =  {69},
  number =  {11},
  pages =   {1556},
  doi =     {10.1063/1.117060},
  issn =    {00036951},
  url =     {http://dx.doi.org/10.1063/1.117060}
}

@article{SamGiao2013,
author = {Sam-Giao, D. and Mata, R. and Tourbot, Gabriel and Renard, Julien and Wysmolek, Andrzej and Daudin, Bruno and Gayral, Bruno},
doi = {10.1063/1.4775492},
issn = {00218979},
journal = {J. App. Phys.},
number = {4},
pages = {043102},
title = {{Fine optical spectroscopy of the 3.45 eV emission line in GaN nanowires}},
url = {http://link.aip.org/link/JAPIAU/v113/i4/p043102/s1\&Agg=doi},
volume = {113},
year = {2013}
}

@article{Sarwar2015,
author = {Sarwar, ATM Golam and Carnevale, Santino D and Yang, Fan and Kent, Thomas F and Jamison, John J and McComb, David W. and Myers, Roberto C},
doi = {10.1002/smll.201501909},
issn = {16136810},
journal = {Small},
number = {40},
pages = {5402--5408},
title = {{Semiconductor Nanowire Light-Emitting Diodes Grown on Metal: A Direction Toward Large-Scale Fabrication of Nanowire Devices}},
url = {http://doi.wiley.com/10.1002/smll.201501909},
volume = {11},
year = {2015}
}

@article{Shi2015,
author = {Shi, Xieqing and Peng, Mingzeng and Kou, Jinzong and Liu, Caihong and Wang, Rui and Liu, Yudong and Zhai, Junyi},
doi = {10.1002/aelm.201500169},
journal = {Adv. Electr. Mater.},
number = {12},
pages = {1500169},
title = {{A Flexible GaN Nanowire Array-Based Schottky-Type Visible Light Sensor with Strain-Enhanced Photoresponsivity}},
url = {http://doi.wiley.com/10.1002/aelm.201500169},
volume = {1},
year = {2015}
}

@Article{Toko2015,
  author =  {Toko, Kaoru and Nakata, Mitsuki and Jevasuwan, Wipakorn and Fukata, Naoki and Suemasu, Takashi},
  title =   {{Vertically Aligned Ge Nanowires on Flexible Plastic Films Synthesized by (111)-Oriented Ge Seeded Vapor–Liquid–Solid Growth}},
  journal = {ACS Appl. Mater. Interfaces},
  year =    {2015},
  volume =  {7},
  number =  {32},
  pages =   {18120--18124},
  url =     {http://pubs.acs.org/doi/abs/10.1021/acsami.5b05394}
}

@article{Triplett2014,
author = {Triplett, Mark and Nishimura, Hideki and Ombaba, Matthew and Logeeswarren, V. J. and Yee, Matthew and Polat, Kazim G. and Oh, Jin Y. and Fuyuki, Takashi and L\'{e}onard, Fran\c{c}ois and Islam, M. Saif},
doi = {10.1007/s12274-014-0462-7},
issn = {1998-0124},
journal = {Nano Res.},
number = {7},
pages = {998--1006},
title = {{High-precision transfer-printing and integration of vertically oriented semiconductor arrays for flexible device fabrication}},
url = {http://link.springer.com/10.1007/s12274-014-0462-7},
volume = {7},
year = {2014}
}

@article{Tsakalakos2007,
author = {Tsakalakos, L. and Balch, J. and Fronheiser, J. and Korevaar, B. A. and Sulima, O. and Rand, J.},
doi = {10.1063/1.2821113},
file = {:C$\backslash$:/Users/calabrese/Desktop/Silicon nanowire solar cells.pdf:pdf},
isbn = {0003-6951},
issn = {00036951},
journal = {App. Phys. Lett.},
number = {23},
pages = {233117},
title = {{Silicon nanowire solar cells}},
url = {http://scitation.aip.org/content/aip/journal/apl/91/23/10.1063/1.2821113},
volume = {91},
year = {2007}
}

@article{Weisse2011,
author = {Weisse, Jeffrey M. and Kim, Dong Rip and Lee, Chi Hwan and Zheng, Xiaolin},
title = {Vertical Transfer of Uniform Silicon Nanowire Arrays via Crack Formation},
journal = {Nano Lett.},
volume = {11},
number = {3},
pages = {1300-1305},
year = {2011},
doi = {10.1021/nl104362e},
URL = {http://dx.doi.org/10.1021/nl104362e}
}

@article{Weisse2012,
author = {Weisse, Jeffrey M. and Lee, Chi Hwan and Kim, Dong Rip and Zheng, Xiaolin},
doi = {10.1021/nl301659m},
isbn = {1530-6992 (Electronic)$\backslash$n1530-6984 (Linking)},
issn = {1530-6984},
journal = {Nano Lett.},
number = {6},
pages = {3339--3343},
pmid = {22594496},
title = {{Fabrication of Flexible and Vertical Silicon Nanowire Electronics}},
url = {http://pubs.acs.org/doi/abs/10.1021/nl301659m},
volume = {12},
year = {2012}
}

@Article{Woelz2015,
  author =  {W\"{o}lz, Martin and Hauswald, Christian and Flissikowski, T and Gotschke, Tobias and Fern\'{a}ndez-Garrido, Sergio and Brandt, Oliver and Grahn, H T and Geelhaar, Lutz and Riechert, H},
  title =   {{Epitaxial Growth of GaN Nanowires with High Structural Perfection on a Metallic TiN Film}},
  journal = {Nano Lett.},
  year =    {2015},
  volume =  {15},
  number =  {6},
  pages =   {3743--3747},
  doi =     {10.1021/acs.nanolett.5b00251},
  pmid =    {26001039},
  url =     {http://pubs.acs.org/doi/abs/10.1021/acs.nanolett.5b00251}
}

@Article{Zettler2015,
  author =  {Zettler, Johannes K. and Hauswald, Christian and Corfdir, Pierre and Musolino, Mattia and Geelhaar, Lutz and Riechert, Henning and Brandt, Oliver and Fern\'{a}ndez-Garrido, Sergio},
  title =   {{High-Temperature Growth of GaN Nanowires by Molecular Beam Epitaxy: Toward the Material Quality of Bulk GaN}},
  journal = {Cryst. Growth. Des.},
  year =    {2015},
  volume =  {15},
  number =  {8},
  pages =   {4104--4109},
  doi =     {10.1021/acs.cgd.5b00690},
  url =     {http://pubs.acs.org/doi/abs/10.1021/acs.cgd.5b00690}
}

@article{Zhao2016,
author = {Zhao, Chao and Ng, Tien Khee and Wei, Nini and Prabaswara, Aditya and Alias, Mohd S and Janjua, Bilal and Shen, Chao and Ooi, Boon S},
doi = {10.1021/acs.nanolett.5b04190},
issn = {1530-6984},
journal = {Nano Lett.},
month = feb,
number = {2},
pages = {1056--1063},
title = {{Facile Formation of High-Quality InGaN/GaN Quantum-Disks-in-Nanowires on Bulk-Metal Substrates for High-Power Light-Emitters}},
url = {http://pubs.acs.org/doi/abs/10.1021/acs.nanolett.5b04190},
volume = {16},
year = {2016}
}






